Kalman Filter Auto-tuning through Enforcing Chi-Squared Normalized Error Distributions with Bayesian Optimization

The nonlinear and stochastic relationship between noise covariance parameter values and state estimator performance makes optimal filter tuning a very challenging problem. Popular optimization-based tuning approaches can easily get trapped in local minima, leading to poor noise parameter identification and suboptimal state estimation. Recently, black box techniques based on Bayesian optimization with Gaussian processes (GPBO) have been shown to overcome many of these issues, using normalized estimation error squared (NEES) and normalized innovation error (NIS) statistics to derive cost functions for Kalman filter auto-tuning. While reliable noise parameter estimates are obtained in many cases, GPBO solutions obtained with these conventional cost functions do not always converge to optimal filter noise parameters and lack robustness to parameter ambiguities in time-discretized system models. This paper addresses these issues by making two main contributions. First, we show that NIS and NEES errors are only chi-squared distributed for tuned estimators. As a result, chi-square tests are not sufficient to ensure that an estimator has been correctly tuned. We use this to extend the familiar consistency tests for NIS and NEES to penalize if the distribution is not chi-squared distributed. Second, this cost measure is applied within a Student-t processes Bayesian Optimization (TPBO) to achieve robust estimator performance for time discretized state space models. The robustness, accuracy, and reliability of our approach are illustrated on classical state estimation problems.

==> basic_example.tex <==
\section{Basic Example}
\label{eqn:basic_example}

For practical use, all of our applications consider continuous to discrete transformation with a sample time $\Delta t$. The first example is a 1D tracking system. Consider a robot that moves along a 1D track and receives position measurements
every time step. The system state, 
$\x{} = [x,
\dot{x}]^T$, evolved overtime according tothe  are governed by the linear time invariant model
\begin{equation}
\label{eq:con_sys_model}
\begin{aligned}
\dot{\mathbf{x}}_t &= \mathbf{A} \x{t} + \mathbf{G} \uVec{t} + \mathbf{\Gamma} \vVec{t} \\
\z{t} &= \HM{} \x{t} + \wVec{t}
\end{aligned}
\end{equation}
\noindent where 
\begin{align*}
\mathbf{A} =
\begin{bmatrix}
0 & 1 \\
0 & 0 
\end{bmatrix}, \ \ 
\mathbf{G} =
\begin{bmatrix}
0 \\
1  
\end{bmatrix}, \ 
\HM{} =
\begin{bmatrix}
1 & 0  
\end{bmatrix}, \ 
\mathbf{\Gamma} = 
\begin{bmatrix}
0 \\ 
1  
\end{bmatrix}. \ 
\end{align*}
The inputs to the system are: a control acceleration $\uVec{t}$, additive white Gaussian noise acceleration process $\vVec{t}$ with intensity $\V$, and additive white Gaussian position measurement noise process $\wVec{t}$ with continuous time intensity $\W$. In the measurement part, we assume we only measure the position and in the process part, we assume only the speed has additive noise so $\V$ and $\W$ are both scalars, $\V = v$, $\W = \omega$. The control input is set as $\uVec{t}=2\cos(0.75t)$, it causes the robot to move with a low frequency oscillation. Applying a zero-order hold discretization to this system, we obtain discrete time position and velocity state $\x{\kCur} = [x, \dot{x}]^T$ and the linear time-invariant parameters for eqs. (\ref{eq:dynModel})-(\ref{eq:measModel}), the discrete time system can be computed by the following equation
\begin{equation}
\begin{aligned}
&\F{} = 
e^{\mathbf{A}\Delta t}, \ \
\mathbf{B} = 
\int_{0}^{\Delta t} e^{\mathbf{A} m} \mathrm{d} m, \ \
\R{} =  \frac{\W}{\Delta t}\\
&\Q{} =  \int_{0}^{\Delta t} e^{\mathbf{A}m} \mathbf{\Gamma} \V \mathbf{\Gamma}^T e^{\mathbf{A}^Tm} \mathrm{d} m 
\label{eq:VanLoans}
\end{aligned}
\end{equation}
The discrete time plant is computed using Van Loan's method \cite{BrownHwang2012}. Thus, we can get the discrete system
\begin{equation}
\begin{aligned}
&\F{} = 
\begin{bmatrix}
1 & \Delta t \\
0 & 1
\end{bmatrix}, \ \
\mathbf{B} = 
\begin{bmatrix}
0.5 \Delta t^2 \\
\Delta t
\end{bmatrix}, \ \ 
\HM{} = 
\begin{bmatrix}
1 & 0
\end{bmatrix}\\
&\Q{} = v\begin{bmatrix}
 \frac{1}{3} \Delta t^3 & \frac{v}{1} \Delta t^2 \\
 \frac{1}{2} \Delta t^2 & \Delta t
\end{bmatrix}, \ \ \R{} = \frac{\omega}{\Delta t}
\end{aligned}
\label{eq:covariance_definitions}
\end{equation}
Both the discrete process noise covariance $\mathbf{Q}$ and the observation noise covariance $\mathbf{R}$ are functions of $\Delta{t}$

%\sjj{Can we provide an initial example which illustrates why cnis is required?}\zzc{The result of the 1D tracking system cannot show the Cnis is better... Use Cnis or original Jnis is almost the same for the 1D system. I found the problem that the mean and variance doesn't match when I test the 2D tracking system. If I need to raise an example, I need to introduce the experiment system first...  Finally I answer this question in the last section of the experiment...}

%We can see if we need to calculate the NIS and finally the $\Cnis$, the value of them is highly non-linear with respect to $\Delta t$ besides the continuous noise intensity $\mathbf{W}$ and $\mathbf{V}$. To the best of our knowledge, the relationship between $\Delta t$ and the NIS related cost has never been investigated. 


==> observability.tex <==
\section{System Observability Problem and Solution}
\label{sct:observability}

We illustrate the challenges by exploring the properties of a linear system.
In previous work, when people use a NEES/NIS related metric to optimize the process and observation noise covariance, the effect of sample time is often ignored \cite{8962573},  \cite{ivanov2014evaluating}, \cite{powell2002automated}. In this work, we show that when using the NEES/NIS metric with a certain sample time, some of the noise parameters may not be observable, i.e., we cannot infer the correct parameters according to the cost function minimization. We use the following experiment result to support this conclusion.\\
\indent For practical use, all of our applications consider continuous to discrete transformation with a sample time $\Delta t$. The first example is a 1D tracking system. Consider a robot that moves along a 1D track and receives position measurements
every time step. The system state, 
$\x{} = [x,
\dot{x}]^T$, evolved overtime according tothe  are governed by the linear time invariant model
\begin{equation}
\label{eq:con_sys_model}
\begin{aligned}
\dot{\mathbf{x}}_t &= \mathbf{A} \x{t} + \mathbf{G} \uVec{t} + \mathbf{\Gamma} \vVec{t} \\
\z{t} &= \HM{} \x{t} + \wVec{t}
\end{aligned}
\end{equation}
\noindent where 
\begin{align*}
\mathbf{A} =
\begin{bmatrix}
0 & 1 \\
0 & 0 
\end{bmatrix}, \ \ 
\mathbf{G} =
\begin{bmatrix}
0 \\
1  
\end{bmatrix}, \ 
\HM{} =
\begin{bmatrix}
1 & 0  
\end{bmatrix}, \ 
\boldsymbol{\Gamma} = 
\begin{bmatrix}
0 \\ 
1  
\end{bmatrix}. \ 
\end{align*}
The inputs to the system are: a control acceleration $\uVec{t}$, additive white Gaussian noise acceleration process $\vVec{t}$ with intensity $\V$, and additive white Gaussian position measurement noise process $\wVec{t}$ with continuous time intensity $\W$. In the measurement part, we assume we only measure the position and in the process part, we assume only the speed has additive noise so $\V$ and $\W$ are both scalars, $\V = v$, $\W = \omega$. The control input is set as $\uVec{t}=2\cos(0.75t)$, it causes the robot to move with a low frequency oscillation. Applying a zero-order hold discretization to this system, we obtain discrete time position and velocity state $\x{\kCur} = [x, \dot{x}]^T$ and the linear time-invariant parameters for eqs. (\ref{eq:dynModel})-(\ref{eq:measModel}), the discrete time system can be computed by the following equation
\begin{equation}
\begin{aligned}
&\F{} = 
e^{\mathbf{A}\Delta t}, \ \
\mathbf{B} = 
\int_{0}^{\Delta t} e^{\mathbf{A} m} \mathrm{d} m, \ \
\R{} =  \frac{\W}{\Delta t}\\
&\Q{} =  \int_{0}^{\Delta t} e^{\mathbf{A}m} \mathbf{\Gamma} \V \mathbf{\Gamma}^T e^{\mathbf{A}^Tm} \mathrm{d} m 
\label{eq:VanLoans}
\end{aligned}
\end{equation}
The discrete time plant is computed using Van Loan's method \cite{BrownHwang2012}. Thus, we can get the discrete system
\begin{equation}
\begin{aligned}
&\F{} = 
\begin{bmatrix}
1 & \Delta t \\
0 & 1
\end{bmatrix}, \ \
\mathbf{B} = 
\begin{bmatrix}
0.5 \Delta t^2 \\
\Delta t
\end{bmatrix}, \ \ 
\HM{} = 
\begin{bmatrix}
1 & 0
\end{bmatrix}\\
&\Q{} = v\begin{bmatrix}
 \frac{1}{3} \Delta t^3 & \frac{1}{2} \Delta t^2 \\
 \frac{1}{2} \Delta t^2 & \Delta t
\end{bmatrix}, \ \ \R{} = \frac{\omega}{\Delta t}
\end{aligned}
\label{eq:covariance_definitions}
\end{equation}
Both the discrete process noise covariance $\mathbf{Q}$ and the observation noise covariance $\mathbf{R}$ are functions of $\Delta{t}$\\
\indent We set our groundtruth $v = 1$, $\omega = 0.1$ and $\Delta t = 0.1$. The Monte Carlo simulation number $N = 200$ and system run time $T = 200 \Delta t$. In Figure \ref{fig:tracking1d_gt_dt01} we plot the $\Cnis$ value w.r.t. different $\omega$ and $v$, where $\omega \in [0.01, 0.5]$, $v \in [0.1, 5.0]$. Then in Figure \ref{fig:tracking1d_gt_dt05}, we let $\Delta t = 0.5$, plot the $\Cnis$ value w.r.t. $v$ and $\omega$. Finally, in Figure \ref{fig:tracking1d_gt_dt0105}, we choose an interesting logical opetration: for each pair $[v,\omega]$, $\omega \in [0.01, 0.5]$, $v \in [0.1, 5.0]$, we calculate $\Cnis$ twice, one when $\Delta t = 0.1$ and the other when $\Delta t = 0.5$. We only record the larger $\Cnis$. In Figure \ref{fig:tracking1d_gt_dt01}, the $\Cnis$ in the deep blue area looks similar. To make it clear, we again calculate $lg(\Cnis)$ to make the plot more distinguishable (In this way, $\Cnis$ smaller than 1 and closer to 0 will be negative so that its color is more clear). We get the corresponding Figure \ref{fig:tracking1d_gt_dt01_log}. The red arrow points out the minimum value, which is not around the groundtruth. in Figure \ref{fig:tracking1d_gt_dt05}, there is a deep blue curve, again, we take $lg(\Cnis)$ and get the corresponding Figure \ref{fig:tracking1d_gt_dt05_log}. The red arrow points out the global minimum value. We find that the global minimum $\Cnis$ is quite random when $\Delta t = 0.1$ or $\Delta t = 0.5$ if we try to run the KF and get the $\Cnis$ plot multiple times. This brings us back to Figure \ref{fig:first_img}. For the single sample time, our cost surface minimum is quite stochastic. Thus, when we use an optimization algorithm to search the surface, the possible estimations can be quite random like Figure \ref{fig:first_img}. However, this situation is different in case Figure \ref{fig:tracking1d_gt_dt0105}. The global minimum is always around [0.1,1], which is highlighted from its $log$ Figure \ref{fig:tracking1d_gt_dt0105_log} . It's obvious now the $\Delta t$ influences the cost function distribution. It would be interesting to see the mapping between different $\Delta t$ value and $\Cnis$.\\
%In Figure \ref{fig:tracking1d_gt_dt01}, when $\omega$ is fixed, the $v$ doesn't influence the $\Cnis$ value. In \ref{fig:tracking1d_gt_dt05}, where $\Delta t = 0.5$, the $\omega$ has more impact on the cost function. However, the $\Cnis$ values the deep blue curve (pointed out by those arrows) are still not distinguishable. In Figure \ref{fig:tracking1d_gt_dt0105}, the smallest $\Cnis$ is around the groundtruth $v$ and $\omega$ (where the red arrow points to). It's very clear the $\Delta t$ influence the cost function distribution. It would be interesting to see the mapping between different $\Delta t$ value and $\Cnis$.\\
\begin{figure*} [ht!]
\centering
\subfloat[]{
\includegraphics[width=0.3\textwidth]{figs/dt01_surface.eps}
\label{fig:tracking1d_gt_dt01}
}
\subfloat[]{
\includegraphics[width=0.3\textwidth]{figs/dt05_surface.eps}
\label{fig:tracking1d_gt_dt05}
}
\subfloat[]{
\includegraphics[width=0.3\textwidth]{figs/dt0105_surface.eps}
\label{fig:tracking1d_gt_dt0105}
}
\\
\subfloat[]{
\includegraphics[width=0.3\textwidth]{figs/dt01_surface_log.eps}
\label{fig:tracking1d_gt_dt01_log}
}
\subfloat[]{
\includegraphics[width=0.3\textwidth]{figs/dt05_surface_log.eps}
\label{fig:tracking1d_gt_dt05_log}
}
\subfloat[]{
\includegraphics[width=0.3\textwidth]{figs/dt0105_surface_log.eps}
\label{fig:tracking1d_gt_dt0105_log}
}
\caption{In figure (a), (b), (c), the colorbar shows the value of $\Cnis$. Figures (d), (e), (f) are the $lg(\Cnis)$ value of (a), (b), (c) respectively.  In (a), $\Delta t = 0.1$; In (b), $\Delta t = 0.5$; In (c), we calculate $\Cnis$ at both $\Delta t = 0.1$ and $\Delta t = 0.5$ for each $[v,\omega]$ pair but only pick the larger cost. The red arrow indicates where the $\Cnis$ is the smallest in each plot. We can see that only in (c)/(f) we have a global minima around the groundtruth value $[v=1,\omega = 0.1]$} 
\label{fig:tracking1d_gt_dt_compare}
\end{figure*}
\indent To check the relationship between the sample time and our cost function, again, we set our system groundtruth $v = 1$ and $\omega = 0.1$. For the Kalman filter system, we firstly fix $v = 1$ and evaluate $lg(\Cnis)$ with $\Delta t \in [0.02, 1]$, $\omega \in [0.01, 0.5]$. Then we fix $\omega = 0.1$ and evaluate $lg(\Cnis)$ with $\Delta t \in [0.02, 1]$, $v \in [0.1, 5.0]$. The Monte Carlo simulation number $N = 200$ and system run time $T = 200 \Delta t$. From Figure \ref{fig:tracking1d_gt}, we notice that when the $v$ is fixed to the groundtruth value, we can have a small $\Cnis$ value only when $\omega$ is around 1. A similar phenomenon happens when we fix the $\omega$, $\Cnis$ is small only when $v$ is around 1. The reason is that when both $v$ and $\omega$ are close to the groundtruth value, the Kalman filter covariance matches the truth system whatever the $\Delta t$ is. When one or both of them are very different from the groundtruth value, the cost $\Cnis$ can be relatively large depends on the $\Delta t$. In Figure \ref{fig:tracking1d_gt_a}, when $\Delta t$ is large, for example 1, the $\Cnis$ value changes a lot along with $v$ but when $\Delta t$ is small, for example 0.02, the $v$ becomes trivial to $\Cnis$ value. This phenomenon can be predicted from Eq. \eqref{eq:VanLoans}. According to Eq. \eqref{eq:VanLoans}, we can see when we increase the $\Delta t$, due to the integral, the $\mathbf{Q}$ gets larger, which means if the $v$ is far from the groundtruth value, its negative impact on the system will be enlarged. This negative impact results in a larger $\Cnis$ value because the Kalman filter can no longer predict correctly due to the wrong process noise covariance. Apparently, when $\Delta t$ is small, the integral is negligible so we can see in Figure \ref{fig:tracking1d_gt_a} the $\Cnis$ is almost consistent when $\Delta t$ is small. The measurement noise covariance has exactly the opposite impact on the system because in Eq. \eqref{eq:VanLoans} the $\mathbf{W}$ is divided by $\Delta t$. This means when $\Delta t$ is small, the measurement noise will have a larger influence on the system, vice versa. That's why Figure \ref{fig:tracking1d_gt_a} and Figure \ref{fig:tracking1d_gt_b} are kind of symmetry vertically.
\begin{figure*} [ht!]
\centering
\subfloat[]{
\includegraphics[width=0.45\textwidth]{figs/tracking1d_gt_fix_o_log.eps}
\label{fig:tracking1d_gt_a}
}
\subfloat[]{
\includegraphics[width=0.45\textwidth]{figs/tracking1d_gt_fix_p_log.eps}
\label{fig:tracking1d_gt_b}
}

\caption{Figure (a) fixs $\omega = 0.1$ and plot $v, \Delta t$ verses $lg(\Cnis)$. Figure (a) fixs $v = 1$ and plot $\omega, \Delta t$ verses $lg(\Cnis)$. We can see only when both of $v, \omega$ are around the groundtruth value, the $\Cnis$ is small whatever the $\Delta t$ is.} 
\label{fig:tracking1d_gt}
\end{figure*}

\indent To check if the similar behavior can be applied to other system, we tried two other systems in this work: 2D tracking and mass-spring systems. The system detail is written in experiment section. For now, we just need to note that for the 2D tracking system, we need to optimize four parameters $[v_0,v_1,\omega_0, \omega_1]$, two for process noise and two for the measurement noise. We set the groundtruth as [1,1,0.1,0.1]. Again, we fix three of them and plot the remaining one verses $\Delta t$ and $\Cnis$. $\omega \in [0.01, 0.5]$, $v \in [0.1,5]$ if they are not fixed. $\Delta t \in [0.02, 1]$. From all the subfigures of figure \ref{fig:tracking2d_gt} we can still notice that only when the noise intensity value is around the groundtruth, the $\Cnis$ can remain small no matter how the $\Delta t$ changes. However, comparing to Figure \ref{fig:tracking1d_gt}, the difference between the area outside of the $v=1$ or $\omega = 0.1$ area and inside of the area is smaller. The reason is straightforward, we have four variables and we fix three of them to the groundtruth value so the rest one's impact on the system is relatively small. This result indicates that if the parameters have high dimension, we may not be able to get an accurate result on each element.\\
\begin{figure*} [ht!]
\centering
\subfloat[]{
\includegraphics[width=0.22\textwidth]{figs/tracking2d_fix_gt_var_p0_log.eps}
\label{fig:tracking2d_gt_a}
}
\subfloat[]{
\includegraphics[width=0.22\textwidth]{figs/tracking2d_fix_gt_var_p1_log.eps}
\label{fig:tracking2d_gt_b}
}
\subfloat[]{
\includegraphics[width=0.22\textwidth]{figs/tracking2d_fix_gt_var_o0_log.eps}
\label{fig:tracking2d_gt_c}
}
\subfloat[]{
\includegraphics[width=0.22\textwidth]{figs/tracking2d_fix_gt_var_o1_log.eps}
\label{fig:tracking2d_gt_d}
}
\caption{In subfigure (a), $v_0 \in [0.1,5]$ while $[v_1, \omega_0, \omega_1]$ use groundtruth value. We apply the same rule to the other subfigures. (a) and (b) look identical because $v_0$ and $v_1$ have the same influence on the system, so do (c) and (d). Again, only when the changing value is around the groundtruth, the $\Cnis$ is small and smilar no matter how the $\Delta t$ changes.} 
\label{fig:tracking2d_gt}
\end{figure*}
\indent We also verify the mass-spring system shares the same property. But for simplification, we'll only show its noise optimization result in section \ref{sct:result}. In all, by leveraging different sample time, the observability of the system can be greatly improved \nra{note to self: edit} (In practice, the system can not be accurately observable, so we don't expect to have an estimation that is the same as the groundtruth, which result in the requirement of covariance consistency Eq. \eqref{eq:cov_consistency}). The take-home message of this section is that the cost function value $\Cnis$ is influenced not only by the noise intensity but the sample time. Only when the noise parameters are around the ground truth, the $\Cnis$ won't be affected much by the sample time. This conclusion, along with NIS theory and BO introduced in the next section builds our optimization strategy.
% where the inputs to the system now consist of a discretized zero-order hold control acceleration $\uVec{\kCur}=2\cos(0.075\kCur)$, additive white process noise vector $\vVec{\kCur} \in \mathbb{R}^2$ with discrete time covariance $\Q{\kCur} \in \mathbb{R}^{2 \times 2}$, and additive white measurement noise $\wVec{\kCur}$ with discrete time covariance $\R{\kCur}$. 
% Note that, given $\V$ and $\W$, the corresponding discrete time noise covariances are 
% %%time invariant values of $\Q{\kCur}$ and $\R{\kCur}$ are 
% \begin{align}
% \R{} &=  \frac{\W}{\Delta T}, \\
% \Q{} &=  \int_{0}^{\Delta t} e^{\mathbf{A}v} \mathbf{\Gamma} \V \mathbf{\Gamma}^T e^{\mathbf{A}^Tv} \Delta v 
% \end{align}
% where the matrix expression for $\Q{}$ can be computed from $\mathbf{A}$, $\mathbf{\Gamma}$, $\V$, and $\Delta T$ using Van Loan's method \cite{BrownHwang2012}. If $\A$ and $\Gamma$ are both known, then this relationship also allows us to design a full $2 \times 2$ positive definite symmetric covariance matrix $\Q{}$ by tuning the corresponding scalar continuous time process noise acceleration intensity $\V$ only.

==> scrap.tex <==


\sijucomm{Existing discussion down here}

We assume if $\Jnees \approx 0$ then the NEES is $\chi^2$ distribution since its mean value equals the $\nx$. However, the $\chi^2$ distribution is not guaranteed. We need to recall the initial reason that researchers try to use $\Jnees$. We define \cite{Bar-Shalom2001}
\begin{equation}
    \mathbf{u} = \covCond{k}{k} ^{-1/2} \mathbf{\ex{k}}
\end{equation}
If the filter is well tuned, i.e, it is unbiased and sufficient.
\begin{equation}
\begin{aligned}
\E{\ex{k}} & = \mathbf{0}, \ \forall k \\
\E{\ex{k}\ex{k}^T} &= \covCond{k}{k}, \ \forall k \\
\ex{k} & \sim {\cal N}(\mathbf{0},\covCond{k}{k})
\end{aligned}
\end{equation}
Each element in $\mathbf{u} = [u_0,u_1...,u_n]$ has standard normal distribution $u_i \sim \mathcal{N}(0,1)$ because 
\begin{equation}
\begin{aligned}
\E{\mathbf{u}} & = \E{\ex{k}} = \mathbf{0}\\
\E{\mathbf{u}\mathbf{u}^T} & = \covCond{k}{k} ^{-1/2} \E{\ex{k}\ex{k}^T}\covCond{k}{k} ^{-1/2} = \mathbf{I}
\end{aligned}
\end{equation}
Thus
\begin{equation}
    \mathbf{U} \doteq \mathbf{u} \mathbf{u}^T = \sum_{i}^{n}u_i^2
\end{equation}
is the square sum of the standard normal distribution, which results in a $\chi^2$ distribution that has mean $\nx$. However, if the filter is not well tuned, each element is just a general normal distribution $u_i \sim \mathcal{N}(m_i, \sigma_i^2)$. The squared sum of a normal distribution with a mean $m$ and unit variance leads to non-central $\chi^2$ distribution. We write it as
\begin{equation}
    u^2 \sim \mathcal{X}(d,\lambda)
\end{equation}
where $d$ is the degree of freedom which is 1 for a normal distribution with a single variable. $\lambda$ is non-centralities and $\lambda = m^2$ \cite{johnson1995continuous}. \hjb{This does not make sense and needs to be revisited.} \zzc{non-central chi square distribution non-centrality equals to the mean squared sum of the unit variance gaussian distribution. This can be seen in the reference I add here}
Specifically, if the normal distribution doesn't have unit variance then its square sum is scaled by its variance 
\begin{equation}
\begin{aligned}
    &\frac{u^2}{\sigma^2} \sim \mathcal{X}(d,\lambda)\\
    &\Longrightarrow u^2 \sim \sigma^2 \mathcal{X}(d,\lambda)
\end{aligned}
\end{equation}
The square sum of the weighted non-central $\chi^2$ function gives the generalized chi-squared distribution.
\begin{equation}
\begin{aligned}
    \mathbf{U} = \sum_{i}^n \sigma_i^2 \mathcal{X}_i(d_i,\lambda_i)
\end{aligned}
\end{equation}
The expectation and variance of the above generalized chi-squared distribution can be given by
\begin{equation}
\label{eq:mean_var_gchi}
\begin{aligned}
    \E{\mathbf{U}} & = \sum_i^n \sigma_i^2(d_i+\lambda_i) \\
    \E{\mathbf{U}\mathbf{U}^T} & = 2\sum_i^n \sigma_i^4(d_i+2\lambda_i) \\
\end{aligned}
\end{equation}
If the filter is unbiased and sufficent, we have the $\chi^2$ distribution constructed by standard normal distributions because $\lambda_i = 0$ and $\sigma_i = 1$. Given $\E{\mathbf{U}} = \nx$ as constraint, i.e., using $\Jnis$ as the cost function, $\lambda_i = 0$ and $\sigma_i = 1$ are just one of the infinite solutions of Eq.\eqref{eq:mean_var_gchi}. In our proposed method, we add the variance into the cost function, i.e, we add the following constraints
\begin{equation}
\begin{aligned}
    \E{\mathbf{U}} & \approx \nx \\
    \E{\mathbf{U}\mathbf{U}^T} & \approx 2\nx \\ 
\end{aligned}
\end{equation}
We show in our experiments that, by adding one more constriants into the cost function, we can significantly increases the robustness of the parameter tuning.




%\crh{For Zhaozhong: Make sure that we discuss CNIS as using multiple dt values. Not currently mentioned.} %zzc{add a simple discription in the above section}




\noindent where 
\begin{align*}
\mathbf{A} =
\begin{bmatrix}
0 & 1 \\
0 & 0 
\end{bmatrix}, \ \ 
\mathbf{G} =
\begin{bmatrix}
0 \\
1  
\end{bmatrix}, \ 
\HM{} =
\begin{bmatrix}
1 & 0  
\end{bmatrix}, \ 
\boldsymbol{\Gamma} = 
\begin{bmatrix}
0 \\ 
1  
\end{bmatrix}. \ 
\end{align*}
The inputs to the system are: a control acceleration $\uVec{t}$ with additive Gaussian white noise and acceleration process $\vVec{t}$ with intensity $\V$, and additive white Gaussian position measurement noise process $\wVec{t}$ with continuous time intensity $\W$. We only measure position in the measurement stage and assume only the speed has additive noise in the process stage which makes $\V = v$, $\W = w$ and $\V$ and $\W$ are both scalars. We apply a low frequency oscillation $\uVec{t}=2\cos(0.75t)$ as the control input.
After applying a zero-order hold discretization to this system, we obtain a discrete time position and velocity state $\x{\kCur} = [x, \dot{x}]^T$ and the linear time-invariant parameters for Eqs. (\ref{eq:dynModel})-(\ref{eq:measModel}), the discrete time system can be computed by the following equation:
